3DN: 3D Deformation Network

Applications in virtual and augmented reality create a demand for rapid creation and easy access to large sets of 3D models. An effective way to address this demand is to edit or deform existing 3D models based on a reference, e.g., a 2D image which is very easy to acquire. Given such a source 3D model and a target which can be a 2D image, 3D model, or a point cloud acquired as a depth scan, we introduce 3DN, an end-to-end network that deforms the source model to resemble the target. Our method infers per-vertex offset displacements while keeping the mesh connectivity of the source model fixed. We present a training strategy which uses a novel differentiable operation, mesh sampling operator, to generalize our method across source and target models with varying mesh densities. Mesh sampling operator can be seamlessly integrated into the network to handle meshes with different topologies. Qualitative and quantitative results show that our method generates higher quality results compared to the state-of-the art learning-based methods for 3D shape generation. Code is available at github.com/laughtervv/3DN.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Applications in virtual reality, augmented reality, and robotics applications require rapid creation and access to large number of 3D models. Promising results have been achieved for shape generation and 3D reconstruction using 3D deep learning techniques. However, performance of these results lags far behind traditional graphics methods and cannot satisfy industrial application requirements. For example, as is shown in Figure~\ref{fig:currentlimitation}, Groueix et al~\cite{groueix2018} and Wang el al~\cite{wang2018pixel2mesh} seek to generate a fixed-topology mesh surface given an image or a point cloud. These methods suffers from lacking of flexibility to generate various shape from the same topology. Moreover, despite their plausible rendered results, the generated meshes are of low quality and suffers from self-intersection and discontinuous surfaces.

In this paper, our goal is to perform 3D mesh reconstruction from a 2D single image or a 3D point cloud target. To overcome the aforementioned challenges in 3D reconstruction via surface generation, we can use existing high-quality meshes to reconstruct similar target, instead of producing a fixed-topology surface. Consider we have access to a small set of source 3D mesh templates and given an image or a point cloud as target, we want to deform a source mesh from the small template set to reconstruct a new mesh that resembles the target. In this way, the 3D reconstruction problem is transformed into a mesh deformation problem. We develop a novel end-to-end network that takes a source template mesh and a 2D single image (or a 3D point cloud) target and predicts per-vertex offset for source mesh for deformation. 

There are three important considerations for our approach.
\paragraph{Why do we need a source mesh?} There are two advantages of reconstructing from a source mesh over fixed-topology surface generation: 1) our model can use high-quality details residing in source mesh and produce much more visually plausible results. 2) triangle connectivity information is hard to infer from both 2D image and point cloud, and fixed-topology surface generation lacks of flexibility to generate various meshes.  

\paragraph{Why do we need deep neural network?} Traditional graphics method requires long pipeline optimization~\cite{qixing,kaixu} and tuning parameters for each sample individually. With the availability of large 3D dataset~\cite{shapenet, s3dis, scannet}, 3D deep learning frameworks~\cite{pointnet, pointcnn, graphnet} open up more efficient and flexible way handle 3D data. We believe these 3D deep learning techniques and large dataset are able to overcome the aforementioned difficulties in traditional computer graphics.

\paragraph{How do we use mesh triangle information and propagate features in network?} Based on the pioneering works in 3D point cloud~\cite{pointnet,pointnet++}, we incorporate mesh sampling operator into network. When a point is sampled from a mesh triangle, both vertices information and geometry in triangles will be integrated and this operation is differentiable. Moreover, we designed a simple architecture to transform source points field to a smooth deformation offset field.

Our pipeline firstly extract global features for both source and target and feed the global features into an offset decoder. The offset decoder takes mesh vertices as input and output per-vertice offset. By adding the offsets, the source mesh is deformed to the target model. Various losses are designed to measure shape similarity and reduce self-intersection in deformation.

We evaluate our framework on both CAD dataset~\cite{shapenet} and real images. Qualitative and quantitative comparison demonstrate that our model is able to reconstruct high-quality mesh without losing similarity information. We also demonstrate the potential of our methods for several applications, such as shape generation and shape interpolation.
%The main contributions of this paper are
%\begin{itemize}
%\item 
%\end{itemize} 

%There are several 
